Discourse Context Predictability Effects in Hindi Word Order

We test the hypothesis that discourse predictability influences Hindi syntactic choice. While prior work has shown that a number of factors (e.g., information status, dependency length, and syntactic surprisal) influence Hindi word order preferences, the role of discourse predictability is underexplored in the literature. Inspired by prior work on syntactic priming, we investigate how the words and syntactic structures in a sentence influence the word order of the following sentences. Specifically, we extract sentences from the Hindi-Urdu Treebank corpus (HUTB), permute the preverbal constituents of those sentences, and build a classifier to predict which sentences actually occurred in the corpus against artificially generated distractors. The classifier uses a number of discourse-based features and cognitive features to make its predictions, including dependency length, surprisal, and information status. We find that information status and LSTM-based discourse predictability influence word order choices, especially for non-canonical object-fronted orders. We conclude by situating our results within the broader syntactic priming literature.

==> rebuttal.tex <==
\pagebreak
\section*{Response to Area Chair and Reviewers}\label{sect:resp}

%Mention the page, paragraph, and line number of any revisions that are made.

We are grateful for the detailed comments from all the four reviewers and the area chair. The subsections in this document provide point-by-point responses to the comments of the area chair and each of the reviewers (comments are italicized). We provide section numbers, page numbers, and pagewise line numbers for each change effected. For greater accuracy, we use a specialized latex package for this purpose. 

\subsection*{Response to Area Chair}

Responses to comments by the area chair are provided below.

\begin{enumerate}

\item {\it This paper focuses on psycholinguistic questions of discourse and priming in Hindi. The paper is not a good fit for the ACL 2022 Special Theme, but may be a good fit for another ACL 2022 session such as Psycholinguistics or Syntax.\\~\\ Hindi is neither a low-resource language nor an endangered language. While Hindi certainly has less in the way of NLP resources than English does, it is highly inappropriate to state that Hindi is a low-resource language.}\\
~\\
With our submission, we intended to highlight the relative lack of linguistically-annotated resources in Hindi (unlike English), which are crucial for theoretically motivated hypothesis-driven research. For example, Hindi does not have any phrase-structure treebank and has just one dependency treebank. For this project, we needed to create essential tools to even work with Hindi, as well as refining and validating syntactically annotated test datasets. In addition to our data, we plan to publicly release all the models and tools we developed to promote future research on Hindi:

\begin{enumerate}
    \item We developed/configured several tools to process Hindi {\it viz.,} tokenizer, tagger, and parser, and obtained syntactic training data.
    \item We developed a Hindi dependency-constituency converter amenable for parser training (not trivial for Hindi) and trained a Hindi incremental PCFG parser.
    \item We annotated our testing corpus semi-automatically for information structure influences.
    % \item We trained a Hindi incremental PCFG parser.
    \item We trained multiple Hindi LSTMs (the only thing that did not require new linguistic annotations or new corpus tools).
\end{enumerate}

However, we do acknowledge the point made, and as suggested, we would like to commit the revised paper to the track --- {\it Linguistic Theories, Cognitive Modeling and Psycholinguistics}. We have also removed our claim about ``Hindi being a low-resource language'' in the revised submission.

\item {\it The constructed experimental data and corresponding results assume that permuted word order is dispreferred to original word order, but do not validate this with human speakers.}

We thank everyone on the reviewer panel for this suggestion. In the revised version, we have validated our findings with human evaluation. We conducted a forced-choice rating task and collected sentence preferences for randomly selected 167 reference-variant pairs from 12 Hindi native speakers. Overall, 89.92\% of the reference sentences which originally appeared in the HUTB corpus were preferred by native speakers compared to the artificially generated grammatical variants expressing similar meanings. The newly added Section \ref{subsec:human-eval} elaborates upon these findings factoring in the feedback pertaining to the human evaluation of word order preferences.

\item \textit{Further description of the corpus would strengthen the paper.}

Section \ref{sect:method}, \lr{AC-hutb} provides further details about HUTB corpus. %In a recent study, \citet{cog:sid} also presents a detailed descriptive analysis of the HUTB corpus.

\item \textit{Authors should examine corpus for breakdown in spoken vs written data.}

For training trigram and LSTM language models, we only use the written section of EMILLE corpus to match the modality of our HUTB test data set faithfully. \lr{AC-hutb} in Section \ref{sect:method} and subsequently, \lr{ac-emille1} and \lr{ac-emille2} in Section \ref{subsect:model} mention these details. Due to space limitations, we do not present the distribution of spoken and written sentences of EMILLE corpus in the main paper, but we present it here as a response. Table \ref{tab:emille-distr} presents the construction distribution of written and conversational sentences in the EMILLE corpus. 

\begin{table}
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Constructions} & \textbf{Written (\%)} & \multicolumn{1}{l|}{\textbf{Conversational (\%)}} \\ \hline
Canonical & 13.22 & 13.67 \\
Non-canonical (DO/IO-fronted) & 2.75 & 2.27 \\
DO-fronted & 1.87 & 1.55\\
IO-fronted & 0.89 & 0.72\\
Subject drop & 41.28 & 43.29 \\
Object (DO/IO) drop & 43.98 & 41.88 \\ \hline
\end{tabular}
\caption{Hindi construction distribution in EMILLE corpus (written: 598086, conversational: 35235 sentences)}
\label{tab:emille-distr}
\end{table}


\item \textit{Additional analysis of adaptive vs vanilla LSTM results are needed.}

We have done exhaustive error analysis in this vein (refer to Appendix E, F, G, H, I), demonstrating where/how the adaptive LSTM surprisal is doing better than a vanilla LSTM. %We have emphasized these observations more in the main text.

\end{enumerate}
  
%We also like to note that where applicable, we have taken the area chair's comments into account in replying to the reviewer's remarks.

\subsection*{Response to Reviewer~1}

\begin{enumerate}
\item {\it The dataset relies on several assumptions about the automatically-created negative data:}

\begin{itemize}

\item {\it \textbf{First}, it assumes that any word order other than the naturally-occurring one is less preferred. If many counterfactual word orders were actually equally preferred, then the features that discriminate between real and counterfactual word orders would not tell us about the correlates of word order preference, but rather the correlates of the counterfactual generation procedure.}

\item {\it \textbf{Second}, it assumes that ungrammatical counterfactual sentences can be automatically filtered by identifying unattested sequences of dependency arcs. If this assumption is wrong, then highly predictive features could just be distinguishing acceptable and unacceptable sentences, rather than the appropriateness of a possible sentence in a discourse context.}

\item {\it Both these limitations could be addressed by doing some human validation of the automatically generated data.}

\end{itemize}

  We concede both the points made by the reviewer. We have now conducted the human evaluation of reference-variant preferences. These new findings are reported in Section \ref{subsec:human-eval}.

\item {\it {The paper repeatedly phrases claims using causal language (e.g. describing which features ``drive'' word order), while the results are essentially correlational.}}

We have replaced the word ``drive'' with ``influence'' throughout the paper.

\item {\it Section 2.1 How is surprisal hypothesized to be related to word order preferences?}

Section \ref{subsect:surp} \lr{R1-surp} cites a couple of works in the literature where researchers have shown that surprisal accounts for word order preferences owing to increased accessibility of multi-word sequences~\citep{arnold:2011festschrift,realiChristiansen2007}. We hypothesize that sentences that originally appeared in the corpus are more accessible than artificially generated variants either due to discourse context or frequent structures. We elaborate more on this in the discussion section \ref{sect:disc}.

\item {\it Ln 188: If the same reference sentence appears multiple times in the dataset, isn’t there a danger that the model will strongly overfit to features of the specific reference sentences?}

No. That is not how we approach the syntactic choice problem in this work. We set up a binary classification task to distinguish if the sentence belongs to a reference sentence category (originally occurred in the HUTB corpus) or artificially generated variants. Our data set contains 1996 reference sentences and 72833 variant sentences. However, to alleviate the imbalance for the classification task, we transform our dataset using \citet{Joachims:2002} technique originally proposed for ranking web pages. This technique converts a binary classification problem into a pair-wise ranking task involving the feature vectors of a reference sentence and each of its variants. As described in Section \ref{subsect:model}, \lr{R1-joc}, We create ordered pairs involving feature vectors of $reference-variant$ and $variant-reference$ and then encoded them as 1 and 0 respectively resulting in a balanced data set. The overall goal is to model two-alternative choices for each reference sentence such that the speaker generated the reference sentence after rejecting a potential grammatical variant. Moreover, the reference sentence that appeared originally in the corpus must have been present due to its properties (viz., discourse context, accessibility, or surprisal), and variant sentences are less likely to be produced due to the same reasons. \citet{cog:raja} has also used this approach to investigate the syntactic choice problem in English.

\item {Ln 211: What does delta mean? Reference sentence minus context sentence?}

Delta ($\delta$) means the difference between feature vectors of the reference sentence and its paired variant. We have also illustrated how we do Joachims transformation in Appendix \ref{appendix:joc} and also pointed in Section \ref{subsect:model}, \lr{R1-joct} of the revised submission.


\item {\it Ln 253: This probably underestimates givennes, because more kinds of expressions can be given: coreferring expressions (e.g. “the first man to walk on the moon” and “Neil Armstrong”), and bridged expressions (e.g. “I walked in the house. The door was open.”)}

We agree with the point made. Since this is one of the first studies that investigated the impact of givenness on word ordering quantitatively, we limit the scope of givenness in the current work and just consider identical content word repetition in subject or object phrase and if content word repetition leads to the fronting of subject/object phrases.

\item {\it Ln 358: Does this result indicate that dependency length is often in conflict with (and overridden by) other factors like discourse and priming? If so, then word order preferences could be seen as an attempt to jointly optimize multiple independent factors.}

This is an exciting suggestion. We concede this possibility in \lr{R1-locality} of subsection \ref{lex:reg} of the revised paper and acknowledge the reviewer in the footnote of the same page. 

% \item {\it Ln 376: An example would make this easier to follow}

\item {\it Adaptive LSTM surprisal (i.e. updating LM weights on successive sentences at test time) is interpreted here (and elsewhere in the paper) as indicative of syntactic priming, while ordinary LSTM LM surprisal is not. Is there a good reason to think that ordinary LSTMs could not show some effect like syntactic priming?}

% We do not claim that adaptive LSTM surprisal is susceptible to only syntactic priming. Instead, we show that adaptive LSTM surprisal captures both vocabularies as well as syntax following the findings also reported by \citet{van2018neural}; thus exhibiting both lexical as well as syntactic priming. We confirm this using ablation study involving entire dataset (see Table \ref{tab:lex-adapt-pred-acc}). We observe that adaptive LSTM surprisal significantly boosts the classification accuracy over and above the baseline model if lexical repetition surprisal is not part of the baseline. This suggests that LSTM adaptation encapsulates both lexical repetition as well as syntactic priming. Besides, syntactic priming was explicit only in non-canonical constructions (IO/DO fronting), where all the surprisal models, including LSTM and lexical repetition surprisal failed to demonstrate their effects.

This is an interesting point. We do agree that ordinary LSTMs could show certain priming effects. More recently, \citet{misra2020exploring} demonstrated that BERT exhibits ``priming effect'' such that the LM was able to predict a word with greater probability when the context included a related word than an unrelated word. However, the effect decreases as the amount of information provided by the context increases. In other words, the related prime under high contextual constraint starts acting as distractor---actively demoting the target word in the probability distribution; thus exhibiting ``mispriming effect''~\cite{kassner-schutze-2020-negated}. This could be due to stylistic avoidance of repeated structures/words in the adjacent sentences. These thoughts are beyond the scope of this paper. In this work, sentences are treated as independent while estimating their surprisal using vanilla LSTM LM, so there is no way vanilla LSTM can exhibit syntactic priming given the independent sentences.

\item {\it {Table 5: Does this analysis deserve so much space? Only one result here is significant, and the effect sizes are very small.}}

Our goal was to conduct exhaustive experimentation and report all the results else this would exacerbate ``file-drawer problem'' in academic publishing. If recommended, we would streamline the result in the main paper and report the rest in the appendix section.

\item {\it Ln 895: Is Hindi strictly verb final? How do you know that arguments won’t appear after the verb?}

Hindi is not a strictly verb-final language but the majority of the constituents in the HUTB corpus are preverbal. Our corpus analysis of 13274 sentences present in HUTB suggests 20,750 pairs of preverbal constituents and 2599 pairs of postverbal constituents. Therefore, our variant generation (via reordering of constituents) and subsequent experiments focus on word-order variation in the preverbal domain, considering preverbal domain to be the locus of word order variation. We permute only preverbal constituents to generate grammatical variants and leave the postverbal constituents in the reference-variants sentences as it is.

\item {\it Ln 84: Make it clear that this claim is about your model, not humans}

We are claiming the syntactic choice preference by humans, which we are trying to capture using a computational model. Please note that reference sentences originally belong to the HUTB corpus generated by a human after eliminating potential variants expressing similar meaning. The model depicts that the reference sentence that appeared originally in the corpus must have been present due to its properties (viz., discourse context, accessibility, or surprisal), and variant sentences are less likely to be produced due to the same reasons.

\item {\it Ln 901: Put the 7 after the comma, so this doesn’t read as 100^7}

This issue has been fixed in the revised version.

\end{enumerate}


\subsection*{Response to Reviewer~2}

\begin{enumerate}
    \item {\it For one, the authors do not describe either of the corpora they have used. Roughly 3\% of the EMILLE corpus for Hindi is spoken transcriptions; is there a difference in the likelihood of non-canonical word orders in spoken vs. written corpora?}

    For training trigram and LSTM language models, we only use the written section of EMILLE corpus to faithfully match the modality of our HUTB test data. \lr{AC-hutb} in Section \ref{sect:method} and subsequently, \lr{ac-emille1} and \lr{ac-emille2} in Section \ref{subsect:model} mention these details. Due to space limitations, we do not present the distribution of the spoken and written sentences of the EMILLE corpus in the paper but present it here as a response. Table \ref{tab:emille-distr} presents the construction distribution of written and conversational sentences in the EMILLE corpus. The distribution of non-canonical word orders is very similar in the spoken (2.27\%) vs. the written (2.75\%) section of the corpus.
    
    \item {\it \hl{Next, it is very unclear why the authors used LSTMs at all. The authors claim that this is to model discourse-level phenomenon, but an LSTM is not inherently a discourse model (indeed, the correlation to trigram features in the Appendix seems to indicate that the LSTM is not learning discourse features).}}
    
    \item {\it Finally, given that this was submitted to the theme track, a significant issue with the paper is that Hindi is neither endangered, nor under-resourced, nor typologically distinct.}
    
    We have fixed this issue with the current version of the paper. We have also removed our claim about ``Hindi being a low-resource language'' in the revised submission.
    
\end{enumerate}

\subsection*{Response to Reviewer~3}

\begin{enumerate}
    \item {\it Effects for most features investigated seem to not be very strong (see table 2)}
    
    We show the effect of adaptation on word order beyond a very competitive and powerful baseline.
    
    \item {\it Is Hindi really a low-resource language?}
    
    We have fixed this issue with the current version of the paper. We have also removed the claim about ``Hindi being a low-resource language'' in the revised submission.
    
\end{enumerate}

\subsection*{Response to Reviewer~4}

\begin{enumerate}
    \item {\it In general, I am not quite sure that this paper fits the theme of "Language Diversity: from Low Resource to Endangered Languages". Per the guidelines provided by ARR, it seems that it fits rather within the realm of "regular papers", which "[address] a specific aspect and/or language with detailed solutions and evaluations".}
    
    We have fixed this issue with the current version of the paper. We have also removed our claim about ``Hindi being a low-resource language'' in the revised submission.
    
    \item {\it Beyond this, I am not sure if the results attested in the paper can be so strongly interpreted as to mean that "word order preferences are driven by lexical and syntactic priming", etc. For example, though the authors demonstrate that adaptive LSTM suprisal improves fit over the baseline variables, it is clear that it is perfectly correlated with basic LSTM surprisal and offers virtually the same classification accuracy. I believe more discussion/analysis should be devoted to how the adaptive LSTM model actually provides substantively different predictions than the vanilla LSTM.}
    
    Appendices \ref{appendix:io-fronting} and \ref{appendix:k1k2k4} already present the error analysis via linguistic examples demonstrating how adaptive LSTM surprisal correctly predicts reference sentence but not the vanilla LSTM surprisal.
    
    \item {\it On top of this, all other surprisal measures are significant in regression and accurate in classification, which leads one to wonder if predictability is really the driver of ordering preferences.}
    
    Over the entire dataset, the success of all the surprisal measures does indicate that predictability is the driver of ordering preferences. However, it does not deny that priming is also playing a role, as both seem to be related or working in the same direction in the current context of this work. However, our actual claim about the success of adaptation/priming in non-canonical construction is a novel contribution of our work. None of the surprisal measures really perform well on these rare linguistic constructions (frequency of DO-fronted = 1\% and IO-fronted = 0.76\% sentences in HUTB corpus) due to their strong frequency bias. Adaptive LSTM surprisal showed its effect in IO-fronted construction as characterized by a significant boost in the classification accuracy. 
    
    \item {\it The other discourse-related measure, IS score, is hardly discussed and its fit over the baseline model is not mentioned. Furthermore, the accuracy of this measure as a predictor is near the baseline 50\%, which indicates that it is hardly interesting.}
    
    The revised submission reports the goodness of fit for IS score over the baseline model containing all other predictors. So for full dataset, \lr{R4-IS} and for DO-fronted construction, \lr{R4-IS-DOIO} in Section \ref{lex:reg} highlight the likelihood-ratio test. Moreover, the information status metric serves as an important baseline for modeling word-order preferences for prediction accuracy experiments.
    
    \item {\it It would have been nice to learn more about the HUTB domain. Given that the study investigates discourse effects, it is unclear how sentences in the HUTB relate to each other.}
    
    Section \ref{sect:method}, \lr{AC-hutb} provides further details about HUTB corpus.
    
\end{enumerate}




